About maximal antichains in a product of two chains:A catch-all note

We establish one-to-one correspondences between maximal antichains in products of two finite linear orders and other mathematical objects, such as certain alignments of two strings, walks on a grid, lattice paths, words of two or three letters. Leaning on these correspondences, we gather what is known about the number of maximal antichains in products of two finite linear orders and we establish some new results.

==> ntheoremdefs.tex <==
\usepackage[centertags,reqno]{amsmath}
\usepackage{mathtools}
\usepackage[thmmarks,amsmath]{ntheorem}
    \RequirePackage{latexsym}
    \RequirePackage{amssymb}
    \theoremnumbering{arabic}
    \theoremstyle{break}
    \theoremsymbol{}
    \theorembodyfont{\itshape}
    \theoremheaderfont{\normalfont\bfseries}
    \theoremseparator{}
    %theorem, proposition, lemma, corollary, definition
\newtheorem{proposition}{Proposition}
\newtheorem{axiom}{Axiom}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{lemma}{Lemma}
    \theoremheaderfont{\normalfont\bfseries}%\slshape}
    \theorembodyfont{\upshape}
    \theoremsymbol{\ensuremath{\,\,\lrcorner}}
\newtheorem{definition}{Definition}
    \theoremsymbol{\ensuremath{\,\,\Diamond}}
    \theoremheaderfont{\normalfont\bfseries}%\slshape}
    \theorembodyfont{\upshape}
\newtheorem{example}{Example}
    \theoremheaderfont{\normalfont\bfseries}
    \theoremsymbol{\ensuremath{\ \bullet}}
\newtheorem{remark}{Remark}
\newtheorem{remTemp}{Temporary Remark}

\theoremstyle{nonumberbreak}
\theoremstyle{nonumberbreak}
\theorembodyfont{\normalfont}
\theoremsymbol{}
\newtheorem{tbd}{To be Done}
\newtheorem{convention}{Convention}
    \theoremheaderfont{\scshape}
    \theoremsymbol{\ensuremath{\ \Box}}
    \newtheorem{proof}{Proof}
    \newtheorem{pproof}{Partial proof}
    \theoremsymbol{}
    \theoremheaderfont{\normalfont\bfseries}
    \newtheorem{proofoflemma}{Proof of the lemma}
    \theoremsymbol{}
    \theoremheaderfont{\normalfont\bfseries}
    \newtheorem{claim}{Claim}
    \theoremsymbol{\par\hfill Fin Ajout}
    \newtheorem{ajout}{Ajout}
    \theoremclass{LaTeX}
    \newtheorem{question}{Question}

    \makeatletter
\newtheoremstyle{denisproof}%
  {\item[\rlap{\vbox{\hbox{\hskip\labelsep \theorem@headerfont
          ##1\theorem@separator}\hbox{\strut}}}]}%
  {\item[\rlap{\vbox{\hbox{\hskip\labelsep \theorem@headerfont
          ##1\ ##3\theorem@separator}\hbox{\strut}}}]}
\makeatother
\theoremstyle{denisproof}
    \theorembodyfont{\normalfont}
    \theoremheaderfont{\scshape}
\theoremsymbol{\ensuremath{\ \Box}}
\newtheorem{sproof}{Proof}

